AIRCHITECT v2: Learning the Hardware Accelerator Design Space through Unified Representations

Design space exploration (DSE) plays a crucial role in enabling custom hardware architectures, particularly for emerging applications like AI, where optimized and specialized designs are essential. With the growing complexity of deep neural networks (DNNs) and the introduction of advanced foundational models (FMs), the design space for DNN accelerators is expanding at an exponential rate. Additionally, this space is highly non-uniform and non-convex, making it increasingly difficult to navigate and optimize. Traditional DSE techniques rely on search-based methods, which involve iterative sampling of the design space to find the optimal solution. However, this process is both time-consuming and often fails to converge to the global optima for such design spaces. Recently, AIrchitect v1, the first attempt to address the limitations of search-based techniques, transformed DSE into a constant-time classification problem using recommendation networks. In this work, we propose AIrchitect v2, a more accurate and generalizable learning-based DSE technique applicable to large-scale design spaces that overcomes the shortcomings of earlier approaches. Specifically, we devise an encoder-decoder transformer model that (a) encodes the complex design space into a uniform intermediate representation using contrastive learning and (b) leverages a novel unified representation blending the advantages of classification and regression to effectively explore the large DSE space without sacrificing accuracy. Experimental results evaluated on 10^5 real DNN workloads demonstrate that, on average, AIrchitect v2 outperforms existing techniques by 15% in identifying optimal design points. Furthermore, to demonstrate the generalizability of our method, we evaluate performance on unseen model workloads (LLMs) and attain a 1.7x improvement in inference latency on the identified hardware architecture.

==> NOTES <==

- 6 pages + 1 page for ref

- Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.


% Surrogate-based approaches, as utilized in~\cite{mindmapping}, aim to mitigate such limitations by training a differentiable performance prediction model that guides the sampling of design points through input gradient. While this strategy improves sampling efficiency, it still necessitates iterative sample searches and faces difficulties in generalizing across various DSE tasks.

==> contents/05-Discussion.tex <==
\section{Discussion and Challenges}

\subsection{Cost of Misprediction}

==> contents/backup.02-Background.tex <==
\section{Background and Motivation}
\label{sec:background_motivation}
\subsection{Target DSE and ML-based Approaches}
\subsubsection{\textbf{Hardware Resource Allocation}}
The performance of machine learning accelerators for a given tensor computation heavily depends on both (1) the mapping style of tensors, represented as tile size, loop order, and spatially parallel dimension, and (2) the allocated hardware components to utilize, such as number of processing engines (PE) or buffer sizes. This results in a vast design space and various non-trivial DSE tasks, depending on the deployment scenario. One such task is hardware resource allocation, which determines the optimal allocation of hardware resources for a given workload and mapping style as shown in \autoref{fig:dse_overview}. %, especially more complicated on hardware systems with larger and abstract configuration space, such as those modeled by MAESTRO~\cite{maestro}. 

%AIrchitect~\cite{airchitect} addressed this DSE task on systolic arrays, through training an MLP model on dataset generated with Scale-Sim~\cite{samajdar2020systematic} simulator. Extending the same task to more complicated accelerators modeled by MAESTRO~\cite{maestro},
ConfuciuX~\cite{confuciux} takes a searched-based approach to address this task on MAESTRO~\cite{maestro}-modeled accelerator, using RL on coarse-granularity and GA on fine-granularity search. It encodes the workload and mapping inputs into samples that can be navigated using the search mechanisms, with the reward aligned with performance metrics such as runtime. 

Although demonstrating the effectiveness, such search-based methods inevitably require iterating over pools of samples. It not only consumes long time that blocks prompt deployment, but also prone to sample efficiency, i.e. how effective the collected samples are.     %On the other hand, HAT~\cite{hat} applied supervised learning on the identical task to enable constant search time, by training a multi-head attention encoder on a dataset consisting of samples collected by ConfuciuX. 
%On the other hand, HAT, AIrchitect \cite{airchitect} applied supervised learning on the identical task to enable O(1) search time, by training a multi-head attention encoder or MLP.

\begin{figure}[t]
    \centering
        \includegraphics[width=\columnwidth]{figures/challenges.pdf}
    \caption{Prominent challenges on DSE datasets; (a) non-uniform and non-convex landscape (b) long-tailed distribution of data samples over labels. }
    \label{fig:challenge}
    \vspace{-5mm}
\end{figure}

\subsubsection{\textbf{Supervised-learning Based Approach}} To mitigate the shortcoming of search-based methods and enable constant and shorter time inference, training a neural network model to predict the optimal design choice has become a promising alternative. AIrchitect~\cite{airchitect} formulated several DSE tasks on systolic-array (including hardware resource allocation) into a classification problem, where its MLP models output the probability distributions over labels, i.e. encoded design choices. The models are trained with dataset consisting of pairs of given DSE inputs and its accordingly optimal design choice, generated by Scale-Sim~\cite{samajdar2020systematic} simulator. GANDSE~\cite{feng2023gandse} took a generative approach, training a GAN based on training dataset generated from the in-house analytical models for FPGA execution.

Nonetheless, such DSE datasets are inherently challenging to train, which manifest as the design space gets larger and complicated. For instance, \textcolor{red}{similar design points may exhibit abrupt discontinuity of performance values, forming a very non-uniform feature embedding space}. In addition, some universally effective design points are highly favored than those suitable for rare cases, resulting in an imbalanced and long-tailed sample distribution over class labels. \textcolor{blue}{~\autoref{fig:challenge}} visualizes these two challenges shown from our target DSE task and its problem sapce. Although these properties are inherent from DSE domain, the prior works did not address sufficiently. 

Another challenge in this direction is the label space of the DSE. The output head of the model architecture needs to cover large enough label space, to properly predict the final design points. However, many DSE tasks will require the models to have larger head at its end, which inhibit generalization of the supervised approach to larger-scale DSE application. The classification head used by AIrchitect~\cite{airchitect} clearly implies such limitation, while GANDSE~\cite{feng2023gandse} already significantly pruned its label space for one-hot encoding.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/overview.pdf}
    \caption{Overview of \name{}, highlighting (1) multi-head self-attention-based encoder and decoder structure, (2) latent embedding space improved by contrastive learning, and (3) UOV heads combining classification and regression.    }
    \label{fig:overview}
\end{figure}

To address these challenges, there is a need to take a deeper look into the problem formulation, model architecture, and training strategies. The following sections mentioned those our work attend to.

\subsection{ML Techniques as Solutions}

\subsubsection{\textbf{Contrastive Learning}}
Contrastive learning as a technique has been widely adopted in self-supervised settings \cite{fu2022contrastive, cao2022synergistic} and is proven to combat overfitting via regularization against negative samples. This work employs contrastive learning to address the issues stemming from the characteristics of DSE dataset. Due to the nature of DNN hardware acceleration, the design points tend to have very discontinuous distribution and biased to the class of majority, resulting in very non-smooth embedding space. Leveraging the contrastive loss results enables learning a uniform and smooth embedding that can aid the model to better learn the DSE search space and generalize to unseen data.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/uov.drawio.pdf}
    \caption{Intuitive visualization of how the same configuration can be represented for regression, classification and the proposed UOV.}
    \label{fig:uov}
    %\vspace{-5mm}
\end{figure}

\subsubsection{\textbf{Classification vs. Regression}}
AIrchitect\cite{airchitect} model the DSE tasks as a classification problem, predicting the label of optimal design point. However, classification requires a fixed-number of predictable labels, i.e. configurations, thereby limiting the coverage of DSE search space. The classification-only approach is also not scalable, because predicting larger design space will require more classification labels and hence larger model size.

On the other hand, regression-based methods can directly predict the DSE hardware allocation parameters. This is a large and unconstrained learning problem, which can result in larger accuracy degradation. However, regression based methods are highly scalable and can be easily extended to large design spaces without increase in model size.

Inspired by \textcolor{blue}{\cite{ramachandran2023ntrans}}, we propose a unified classification and regression approach to leverage the best of both worlds, which is described \autoref{sec:proposed-model} and \ref{sec:train-method}.

\begin{comment}
We develop \uov{}(Unified Ordinal Vectors), a unified encoding of the model predictions in such a way that classification labels, or \textit{buckets}, are used to represent ranges of DSE points instead of a single configuration. The model learns to simultaneously predict the classification bucket and regress the corresponding configuration within the bucket. That is, we propose to do regression within each classification label that now encodes a range of configurations, rather than the whole DSE range. In this fashion, we address the shortcomings of using either technique independently.
\end{comment}


==> contents/backup.03-Methodology.tex <==
\section{Methodology}\label{sec:method}
Our approach is presented as follows: problem space analysis (\ref{sec:prob-formulation}), proposed model for the learning  (\ref{sec:proposed-model}), and training strategies to handle the DSE-inherent challenges (\ref{sec:train-method}).
\subsection{DSE Problem Formulation}\label{sec:prob-formulation} 

\input{tables/problem-def}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/prob-space.pdf}
    \caption{Complexity of the problem space from \autoref{tab:problem-def}, visualizing the input features ($xy$-plane, processed with PCA) and output configuration labels ($z$-axis). This justifies the need of sophisticated model architecture. }
    \label{fig:prob-space}
    %\vspace{-5mm}
\end{figure}

To translate the hardware resource allocation on ~\cite{maestro}-modeled accelerator into learnable formulation, we encode the parameters adopting and modifying the scheme from ConfuciuX~\cite{confuciux}, as summarized in  \autoref{tab:problem-def}. The tenser dimensions for GEMM operation($M,N,K$) are numerical integer values while dataflow is categorical data chosen among a few representative accelerators: weight stationary (NVDLA~\cite{nvdla}), output stationary (ShiDianNao~\cite{du2015shidiannao}), and row stationary (Eyeriss~\cite{chen2016eyeriss_jssc}). 

The outputs are the optimal hardware resources for the given inputs, configured as the number of PEs and buffer size. The dataset is generated via executing the search-based ConfuciuX~\cite{confuciux}, with the optimization metric chosen as latency.  %Each configuration is encoded into a unique \textit{"Configuration ID"}, which becomes the classification labels for the model.

This problem formulation from ~\autoref{tab:problem-def} results in a large DSE space of size $O(10\textsuperscript{9})$. \autoref{fig:prob-space} shows the complexity of this data space, necessitating advanced neural network training to learn the space instead of simple techniques such as decision tree or small MLP. Furthermore, as shown in \textcolor{blue}{~\autoref{fig:challenge}}, the dataset exhibits highly non-uniform embedding space as well as imbalanced label distribution. The following sections explains our contributions to address the challenges.

\subsection{\name{}: multi-head attention-based model}\label{sec:proposed-model} 
\autoref{fig:overview} describes the overall structure of \name{}, which is inspired by the well-known Transformer~\cite{vaswani2017attention} architecture. \name{} consists of the \textbf{encoder} part, which generates the latent space for DSE input samples, and the \textbf{decoder} part, which produce the predictions of optimal design point by processing the intermediate representation. Both the encoder and decoder parts rely on multi-head attention (MHA) layers to learn the complicated relationship among features.

The encoded input vector(\autoref{tab:problem-def}) gets transformed into an embedding matrix where the encoder's MHA layer applies self-attention operations to capture information and formulate the embedding space. Then, the decoder's MHA layer decodes the intermediate embedding and pass the result to the \uov{} heads (explained in the following section) which generates the final hardware configuration.
 
 %Training is done with cross-entropy loss between the probability distribution and the label. For inference, the predicted configuration ID can be decoded back into the number of PEs and buffer sizes, describing the hardware resources allocation recommended by the model.

\begin{algorithm}[t]
\caption{Ordinal Encoding}\label{alg:enc}
\SetKwInOut{KwIn}{Input}
\SetKwInOut{KwOut}{Output}
\SetKwComment{Comment}{/* }{ */}
\KwIn{Ground-truth DSE-config $ D_{gt} \in \mathbb{R}$, $K$ buckets produced $\Lambda = \{r_0, r_2, ... , r_{K-1}\}$}

\KwOut{Ordinal vectors $\{O_i \in \mathbb{R}\}_{i=1}^K$}

    \For{$i = 0$ to $K-1$}
    {
        \If{$D \geq r_i$}
        { 
            \STATE $O_i \gets 1-\exp^{-|{D - r_i}|}$\;
        }

        \Else
        {
            \STATE $O_i \gets 0 $\;
        }
    }
\Return $\{ O_i \}_{i=1}^K$\
\end{algorithm}

\begin{comment}
\begin{algorithm}[t]
\caption{Ordinal Decoding}\label{alg:dec}
\SetKwInOut{KwIn}{Input}
\SetKwInOut{KwOut}{Output}

\KwIn{Predicted ordinal vectors $\{O_i \in \mathbb{R}_{i=1}^K$, $K$ buckets produced $\Lambda = \{r_0, r_2, ... , r_{K-1}\}$}

\KwOut{Decoded DSE-point $ D \in \mathbb{R}$ }

    \tcp{Select Optimal Index}
    $o \gets \arg \max_{i \in O} O_i$\;

    \tcp{Regress DSE value}
    $ D \gets -\ln(1 - O_o) + r_o$\;
    

\Return $D$\
\end{algorithm}
\end{comment}
\subsection{Training Methodology}\label{sec:train-method} 

The training of \name{} takes place in two stages, each stage involving the encoder block and the decoder block, respectively. Both blocks can be trained simultaneously as long as the gradients from decoder do not propagate to encoder.

\subsubsection{\textbf{Stage 1. Encoder Training}} The encoder takes the input features and encodes it into a feature embedding guided by the contrastive loss and a performance prediction.

\noindent\textbf{Contrastive Learning.} We propose to use the infoNCE loss variant \cite{fu2022contrastive} of contrastive loss, but augment it to balance the positive and negative samples. Our modified contrastive objective can be defined as,
\begin{equation}
\label{equation:contrastive}
    \mathcal{L}^C = -\log \frac{ \sum_{p+}\exp(\lambda^p \cdot \lambda^{p+} / \tau)}{ \sum_{p+} \exp (\lambda^p \cdot \lambda^{p+} / \tau) + \sum_{p-} \exp(\lambda^p \cdot \lambda^{p-} / \tau)}
\end{equation}

where, $\lambda$ is the output latent embedding from the encoder, and p, p+ and p- are the anchor, positive and negative samples typically used in contrastive loss \cite{fu2022contrastive}.

\noindent \textbf{Performance Predictor.}  To add semantic information to the feature embedding, we employ an L1-based performance (i.e. latency in this work) prediction loss, $\mathcal{L}^{perf}$.

The final stage 1 loss can thus be formulated as, 
    
\begin{equation}
    \mathcal{L}^{stage1} = \mathcal{L}^C + \mathcal{L}^{perf}
\end{equation}
The entire stage 1 training will be conducted for 500 epochs to suitably learn the latent feature embedding.


\subsubsection{\textbf{Stage 2. Decoder + \uov{} Head Training}} The decoder that implements \uov{} is trained on a unified, (1) classification formulation for range-buckets and (2) regression for finer-granularity search within the bucket. The final decoder \uov{} prediction is guided by a unified focal loss (explained later) with the ground-truth values. %This stage can either be trained independently or in unison with stage 1 as long as gradient propagations are contained within each stage individually.

\noindent \textbf{Unified Ordinal Vectors. }Our unified approach must enable the model to jointly predict the classification bucket while regressing to the actual DSE configuration within the bucket. Given a DSE range or search space, we employ Space Increasing Discretization \cite{miao2023occdepth} to generate the classification buckets consisting of \textit{ranges} of DSE-points instead of a single point. Assuming a DSE search space is discretized into $K$ discrete buckets, $\Lambda = \{ r_0, r_1, ..., r_{K-1} \}$, each DSE configuration can be represented as a K-length \uov{} such that all values leading to the argmax class are monotonically increasing and are non-zero whereas the remaining elements are zero. Such a unified ordinal representation allows encoding important ordering information and is also most amenable for the model to learn and predict because of its regular structure. The final \uov{} ($O$) formulation can thus be written as,

 
\begin{equation}
\{O_i\}_{i=0}^{K-1}=
\begin{cases}
  1-f(|D - r_i|), & \text{if } D \geq r_i \\
  0, & \text{otherwise}
\end{cases}
\end{equation}

where, D is the particular DSE configuration value either PE size or buffer size we want to encode as a \uov{} and $f$ can be any choice-dependent monotonically increasing function. \autoref{fig:uov} intuitively visualize this process and \autoref{alg:enc} shows shows algorithms we used to encode a DSE configuration to unified ordinal vectors. Decoding the \uov{} back to the actual DSE configuration value is the exact reverse of it.

\textbf{Stage 2 Learning Objective. }We make use of a \textit{Ordinal Focal Loss} ($L_o$) as the primary training loss. Here we discuss the formulation for a certain scale \textcolor{red}{(what does scale means?)}, but while training, the loss is calculated independently for each scale and is aggregated across scales. 

\begin{equation}
    \hspace{-2pt}L_o = \sum_{i=0}^{{K-1}}\hspace{-2pt}
    \begin{cases}
        \alpha|q_i-u_i|^\gamma BCE(u_i,q_i),& \hspace{-5pt} \text{if } q_i > 0 \\ 
        (1-\alpha)u_i^\gamma BCE(u_i,q_i),& \hspace{-5pt} \text{otherwise}
    \end{cases}
\end{equation}

\begin{equation}
 BCE(u_i,q_i)= -q_ilog(u_i)-(1-q_i)log(1-u_i)
\end{equation}
where,  $u,q$ are the predicted and ground-truth \uov{}s respectively, and $\alpha=0.75, \gamma=1$. Using \uov{}s and $L_o$, we are able to naturally encapsulate explicit order relationships among labels while minimizing the \textcolor{blue}{??}. With this formulation, predictions whose ordinal labels lie farther away from the ground-truth label will be penalized more than predicted labels closer to ground-truth along with penalization of the actual likelihood within a predicted class to ensure the correct label is predicted and the correct absolute difference of the actual depth value from each non-zero label is predicted.

%Current classification approach that \name{} employs possess limitation in DSE generalization. Formulating the DSE design points into labels is implausible for many DSE tasks. Even in this target hardware resource allocation problem, the data distribution per labels are extremely imbalanced and sparse(~\autoref{fig:dse}-right). We aim to address such limitations through replacing the classification end with combination of classification and regression, adopting the idea proposed in . 

%This approach is expected to enable extendable  we have the classification head determine coarse-level range of the recommended hardware configuration choices, and have the regression head further determine the exact choice within the coarse-level choice from the classification head.


==> include/cmds.tex <==

\newcommand{\TK}[1]{{\color{blue}\bfseries [TK: #1]}}
\newcommand{\JS}[1]{{\color{teal}\bfseries [JS: #1]}}
\newcommand{\AR}[1]{{\color{green}\bfseries [AR: #1]}}
% Name
% \newcommand{\name}[1]{{{{\textsc{AIrchitect} v2}}}\xspace}

\newcommand{\name}[1]{\textsc{AIrchitect v2}\xspace}



\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}


\newcommand{\uov}[1]{{\textbf{\texttt{UOV}}}\xspace}


==> tables/hyper-param.tex <==
% \begingroup	
% % \setlength{\tabcolsep}{3 pt}
% \begin{table}[t]\centering
%  \caption{Hyperparameter Setting}
% % \vspace{-10pt}
%  % \setlength\tabcolsep{2.0pt}
% \resizebox{0.6\linewidth}{!}{%
% \begin{tabular}{cc}
% \Xhline{2\arrayrulewidth}
% Parameter & Value \\
% \Xhline{1\arrayrulewidth}
% Stage 1 Epochs & 500 \\
% Stage 2 Epochs & 100 \\
% Contrastive Learning $\tau$ & 0.4 \\
%  \Xhline{2\arrayrulewidth}
% \end{tabular}
% }
% %\vspace{-10pt}
% \label{tab:param}
% \end{table}
% \endgroup


% \begingroup	
% % \setlength{\tabcolsep}{3 pt}
% \begin{table}[t]\centering
%  \caption{DSE accuracy comparison against competing methods before milestone period.}
%  \vspace{-10pt}
%  % \setlength\tabcolsep{2.0pt}
% \resizebox{0.7\linewidth}{!}{%
% \begin{tabular}{lc}
% \Xhline{2\arrayrulewidth}
% Model & Accuracy (\%) \\
% \Xhline{1\arrayrulewidth}
% AIrchitect v1 \cite{airchitect} & 77.6 \\
% HAT \cite{hat} & 78.8 \\
% \textbf{AIrchitect v2 (Ours)} & \textbf{89.5} \\
%  \Xhline{2\arrayrulewidth}
% \end{tabular}
% }
% \vspace{-5pt}
% \label{tab:acc}
% \end{table}
% \endgroup

% \begingroup	
% % \setlength{\tabcolsep}{3 pt}
% \begin{table}[t]\centering
%  \caption{AIrchitect v2 final DSE accuracy after implementing all three contributions.}
%  \vspace{-10pt}
%  % \setlength\tabcolsep{2.0pt}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcc}
% \Xhline{2\arrayrulewidth}
% Model & Model Size (\# parameters) & Accuracy (\%) \\
% \Xhline{1\arrayrulewidth}
% AIrchitect v1 \cite{airchitect} & - & 77.6 \\
% HAT \cite{hat} & 730059 &  78.8 \\
% \textbf{AIrchitect v2 (Ours) Cla} & 1586430 & \textbf{89.5} \\
% \textbf{AIrchitect v2 (Ours) Reg + Cla} & 813866 & \textbf{87.1} \\
%  \Xhline{2\arrayrulewidth}
% \end{tabular}
% }
% %\vspace{-5pt}
% \label{tab:acc}
% \end{table}
% \endgroup

% \begingroup	
% % \setlength{\tabcolsep}{3 pt}
% \begin{table}[t]\centering
%  \caption{Accuracy Comparison of {\sc AIrchitect v2} with other learning-based techniques }
%  \vspace{-5pt}
%  % \setlength\tabcolsep{2.0pt}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcc}
% \Xhline{2\arrayrulewidth}
% Model & Model Size (\# parameters) & Accuracy (\%) \\
% \Xhline{1\arrayrulewidth}
% AIrchitect v1 \cite{airchitect} & - & 77.6 \\
% HAT \cite{hat} & 730059 &  78.8 \\
% \textbf{AIrchitect v2 (Ours) Cla} & 1586430 & \textbf{89.5} \\
% \textbf{AIrchitect v2 (Ours) Reg + Cla} & 813866 & \textbf{87.1} \\
%  \Xhline{2\arrayrulewidth}
% \end{tabular}
% }
% %\vspace{-5pt}
% \label{tab:acc}
% \end{table}
% \endgroup



% \mathcal{L}^C + \mathcal{L}^{perf}
% \begingroup	
% % \setlength{\tabcolsep}{3 pt}
% \begin{table}[t]\centering
%  \caption{AIrchitect v2 stage 1 ablations.}
%  \vspace{-10pt}
%  % \setlength\tabcolsep{2.0pt}
% \resizebox{0.7\linewidth}{!}{%
% \begin{tabular}{ccc}
% \Xhline{2\arrayrulewidth}
% $\mathcal{L}^C$ & $\mathcal{L}^{perf}$ & Final Classification Accuracy (\%) \\
% \Xhline{1\arrayrulewidth}
% \xmark & \xmark & 79.43 \\
% \xmark & \cmark & 81.27 \\
% \cmark & \xmark & 86.97 \\
% \cmark & \cmark & \textbf{89.54} \\
%  \Xhline{2\arrayrulewidth}
% \end{tabular}
% }
% %\vspace{-10pt}
% \label{tab:stage1-abl}
% \end{table}
% \endgroup

% \mathcal{L}^C + \mathcal{L}^{perf}
% \begingroup	
% % \setlength{\tabcolsep}{3 pt}
% \begin{table}[t]\centering
%  \caption{AIrchitect v2 stage 2 ablations.}
%  \vspace{-10pt}
%  % \setlength\tabcolsep{2.0pt}
% \resizebox{0.75\linewidth}{!}{%
% \begin{tabular}{lc}
% \Xhline{2\arrayrulewidth}
% Decoder Architecture & Final Classification Accuracy (\%) \\
% \Xhline{1\arrayrulewidth}
% MLP & 82.59 \\
% \textbf{Transformer} & \textbf{89.54} \\
%  \Xhline{2\arrayrulewidth}
% \end{tabular}
% }
% %\vspace{-10pt}
% \label{tab:stage2-abl}
% \end{table}
% \endgroup


% \begingroup	
% % \setlength{\tabcolsep}{3 pt}
% \begin{table}[t]\centering
%  \caption{AIrchitect v2 encoder/decoder number of attention heads.}
%  \vspace{-10pt}
%  % \setlength\tabcolsep{2.0pt}
% \resizebox{0.8\linewidth}{!}{%
% \begin{tabular}{cc}
% \Xhline{2\arrayrulewidth}
% \# Enc/Dec Heads & Final Classification Accuracy (\%) \\
% \Xhline{1\arrayrulewidth}
% 2/2 & 88.61 \\
% 4/4 & 89.03 \\
% 8/8 & 89.54 \\
% 16/16 & 89.56 \\
%  \Xhline{2\arrayrulewidth}
% \end{tabular}
% }
% %\vspace{-10pt}
% \label{tab:attn-heads}
% \end{table}
% \endgroup

==> tables/problem-def-conv.tex <==
\begin{table}[t]
\scriptsize
\centering
\setlength{\abovecaptionskip}{0pt}
%\setlength{\belowcaptionskip}{0pt}
%\scriptsize
\renewcommand{\arraystretch}{1.5}
\caption{Input and output formulations for MAESTRO~\cite{maestro}-based hardware resource allocation, adopted from \cite{confuciux}}
\label{tab:problem-def}
  \begin{threeparttable}[b]
\begin{tabular} {|@{~} c @{~}|c|}
\hline
\multicolumn{1}{|c|}{\textbf{}} &
\multicolumn{1}{c|}{\textbf{Features(max)}} 
\\
\hline

\hline
Input & K(512), C(512), Y(256), X(256), R(9), S(9), dataflow(3)  \\
\hline
Output & Configuration ID(768) $= PE * BUF_{max} + BUF$  \\

\hline
\end{tabular}
 \begin{tablenotes}
     \item[] K=number of filters, C=number of channels, Y/X=height/width of input feature map,  R/S=height/width of filter, dataflow=choice among [\cite{nvdla}, \cite{du2015shidiannao}, \cite{chen2016eyeriss_jssc}]  \\
      
 \end{tablenotes}
 \end{threeparttable}
\vspace{-0.25in}
\end{table}


==> tables/results-input-features.tex <==

\begin{table*}[t]
\begin{tabular}{|c||c|c||c|c|c|c|}
\toprule
Input Feature & \multicolumn{2}{c|}{Stage 0 Loss} & \multicolumn{2}{c|}{Stage 1 Acc} &  \multicolumn{2}{c|}{Stage 1 Acc}\\
  Encoding Scheme & \multicolumn{2}{c|}{(Supervised Contrastive)} & \multicolumn{2}{c|}{MLP-based Decoder } &  \multicolumn{2}{c|}{Transformer Decoder}\\
\cline{2-7}
  
   & w/o pe & w/ pe & w/o pe & w/ pe & w/o pe & w/ pe\\
\hline
   
default \cite{hat} & \textbf{2.22302} & 2.22677 & 77.3&76.62 & \textbf{95.88} & 95.83 \\
O (1.) & 2.28662 & 2.29564 & 76.24&75.35 & 94.97 & 94.59 \\
P (2.) & 2.26128 & 2.26543 &  59.69&76.04 & 95.31 & 95.25 \\
OP (1. + 2.) & 2.24894 & 2.24792 & \textbf{78.56}& 21.29 & 95.36&95.33 \\
\bottomrule
\end{tabular}
\caption{Supervised contrastive loss (for stage 0, trained for 100 epochs) and final training accuracy (for stage 1, trained for 60 epochs) on different input feature schemes. 'O', 'P', and 'OP' corresponds representation of '1.Loop order', '2. Parallel Dimension', and both 1. and 2., as described in \autoref{fig:inp-vec}. 'w/o pe' and w/ pe' stand for without and with positional encoding, respectively. }
\label{tab:inp-feat-train}

\end{table*}

